LiDARTouch: Monocular metric depth estimation with a few-beam LiDAR

Vision-based depth estimation is a key feature in autonomous systems, which often relies on a single camera or several independent ones. In such a monocular setup, dense depth is obtained with either additional input from one or several expensive LiDARs, e.g., with 64 beams, or camera-only methods, which suffer from scale-ambiguity and infinite-depth problems. In this paper, we propose a new alternative of densely estimating metric depth by combining a monocular camera with a light-weight LiDAR, e.g., with 4 beams, typical of today's automotive-grade mass-produced laser scanners. Inspired by recent self-supervised methods, we introduce a novel framework, called LiDARTouch, to estimate dense depth maps from monocular images with the help of ``touches'' of LiDAR, i.e., without the need for dense ground-truth depth. In our setup, the minimal LiDAR input contributes on three different levels: as an additional model's input, in a self-supervised LiDAR reconstruction objective function, and to estimate changes of pose (a key component of self-supervised depth estimation architectures). Our LiDARTouch framework achieves new state of the art in self-supervised depth estimation on the KITTI dataset, thus supporting our choices of integrating the very sparse LiDAR signal with other visual features. Moreover, we show that the use of a few-beam LiDAR alleviates scale ambiguity and infinite-depth issues that camera-only methods suffer from. We also demonstrate that methods from the fully-supervised depth-completion literature can be adapted to a self-supervised regime with a minimal LiDAR signal.

==> figures/teaser/teaser.tex <==
\begin{figure*}[!ht]
\centering

\begin{subfigure}[t]{0.48\linewidth}
\begin{tikzpicture} %[trim axis left, trim axis right]
% manual link https://ftp.cc.uoc.gr/mirrors/CTAN/graphics/pgf/contrib/pgfplots/doc/pgfplots.pdf
%\hspace{12pt}
    \begin{axis}[
        % cycle list https://tex.stackexchange.com/questions/170221/pgfplots-line-colors
        % link to color palette: http://www.traag.net/wp/wp-content/uploads/2014/06/display_colors1.png
        % load a color `cycle list' from the `colorbrewer' library
        legend cell align={left}, % align legend on the left
        cycle list/Set1-3,
        % define fill color for the marker
        mark list fill={.!40!white},
        % create new `cycle list` from existing `cycle list`
        cycle multiindex* list={
            Set1-3
                \nextlist
            my marks
                \nextlist
            [3 of]linestyles
                \nextlist
            very thick
                \nextlist
        },
        xmin=-4, xmax=68,
        ymin=0.8, ymax=19,
        ylabel= RMSE (meters),
        %ylabel near ticks,
        ylabel style={yshift=-15pt},
        ymode=log,
        log ticks with fixed point,
        ytick pos=left,
        xlabel=Number of input LiDAR beams,
        xtick={0,4,8,16,32,64},
        xlabel style={yshift=5pt},
        xtick pos=bottom,
        legend style={draw=none, at={(0.45,1.25)}, anchor=north,legend columns=2,
        %legend style={draw=none, at={(0.5,-0.2)}, anchor=north, legend columns=2,
        font={\small} 
        }, 
        scale only axis,height=4cm,width=0.85\linewidth,
        ]
        
\pgfplotsset{cycle list shift=+17}
\addplot+[solid] plot coordinates {
    (4,     2.5048)
    %(8, )
    (16, 2.2366)
    (64, 1.2622)
};
\addlegendentry{LiDARTouch (self-sup.)}

%\addlegendentry{Our LiDARTouch framework, self-supervised}
% cycle is red blue green
% skip +2 so that next plot is blue
%\pgfplotsset{cycle list shift=+6}
\pgfplotsset{cycle list shift=+3}
\addplot+[solid] plot coordinates {
    (64,    2.4068)
    (32,    12.0147)
    (16,    14.2953)
    (8,     15.6683)
    (4,     15.8803)
};
%\addlegendentry{Depth completion, self-supervised}
\addlegendentry{Depth completion (self-sup.)}

\pgfplotsset{cycle list shift=+4}
\addplot+[only marks] plot coordinates {
    (0,     3.2)
};
%\addlegendentry{Image-only setup, self-supervised.}
\addlegendentry{Image-only (self-sup.)}

\pgfplotsset{cycle list shift=+1}    
\addplot+[densely dashed] plot coordinates {
    (64,    0.998)
    (32,    1.1224)
    (16,    1.3761)
    (8,     1.6573)
    (4,     2.1124)
};
%\addlegendentry{Depth completion, supervised with GT}
\addlegendentry{Depth completion \emph{(sup)}}


\draw [color=black][line width=1]  [pattern={on 1.69pt off 2.76pt}]  (80,0.9) -- (80,2.8) ;
\draw [shift={(80,1.0)}] [color=black][line width=1]   (-10,0.15) .. controls (-5,0.1) .. (0,0) .. controls (5,0.1) .. (10,0.15); % Tip of arrow
\end{axis}
\end{tikzpicture}
\caption{
\textbf{Comparison of LiDARTouch vs.\ depth completion approaches.}
In the depth completion setting, results are highly degraded when the ground-truth depth information is no longer available for supervision (blue plots, \emph{sup} vs.\ self-sup).
However, by combining ideas of the self-supervised monocular depth estimation, along with a careful integration design of the LiDAR, we show that our self-supervised LiDARTouch framework can reach performances very close to the fully-supervised depth completion setting, as illustrated by the black arrow.
Note that the $y$-axis is log-scaled.
}
\label{fig:teaser:depth_completion}
\end{subfigure}%
\hfill
\begin{subfigure}[t]{0.51\linewidth}
%\begin{tikzpicture}[every node/.style={inner sep=0,outer sep=0}, spy using outlines={magnification=7, every spy on node/.append style={thick}}]
\begin{tikzpicture}[every node/.style={inner sep=0,outer sep=0}, spy using outlines={magnification=7, every spy on node/.append style={thick}}]

    %%% INPUT
    \node (FigA) {\includegraphics[width=0.67\linewidth]{figures/teaser_input.pdf}};
    %%% LABEL INPUT
    \node [anchor=east] at ($(FigA.west)$) {\rotatebox{90}{Input image}};
    
    %%% DEPTH IMAGE ONLY
    \node[below=0.05cm of FigA] (FigB) {\includegraphics[width=0.67\linewidth]{figures/teaser_image_only.pdf}};
    %%% LABEL DEPTH IMAGE ONLY
    \node [anchor=east] at ($(FigB.west)$)
    {\rotatebox{90}{\parbox{2cm}{\centering Image-only}}};
    %%% ZOOM DEPTH LIDAR
    \node [anchor=north west, draw=red, ultra thick] (zoomFigB) at ($(FigA.north east)+(0,-0.5)$) {\includegraphics[width=0.28\linewidth]{figures/teaser_image_only_zoom.png}};
    %%% red rectangle
    \node[rectangle, draw=red, ultra thick, size=0.7cm] (rectFigB) at ($(FigB)+(-0.15,0)$) {};
    %%% RED LINE
    \draw[red, ultra thick] (rectFigB) -- (zoomFigB);
    
    %%% DEPTH LIDAR
    \node[below=0.05cm of FigB] (FigC) {\includegraphics[width=0.67\linewidth]{figures/teaser_with_lidar.pdf}};
    %%% LABEL DEPTH LIDAR
    \node [anchor=east] at ($(FigC.west)$) {\rotatebox{90}{\parbox{2cm}{\centering LiDARTouch}}};
    %%% ZOOM DEPTH LIDAR
    \node[anchor=south west, draw=black!20!green, ultra thick] (zoomFigC) at ($(FigC.south east)$) {\includegraphics[width=0.28\linewidth]{figures/teaser_with_lidar_zoom.png}};
    %%% green rectangle
    \node[rectangle, draw=black!20!green, ultra thick, size=0.7cm] (rectFigC) at ($(FigC)+(-0.15,0)$) {};
    %%% GREEN LINE
    \draw[black!20!green, ultra thick] (rectFigC) -- (zoomFigC);
\end{tikzpicture}
\caption{\textbf{Mitigation of the infinite-depth problem.}
Self-supervised image-only approaches tend to predict objects with no relative-motion at an infinite depth, as indicated by the hole in the depth close-up (red).
Instead, thanks to the minimal LiDAR integration, our LiDARTouch framework correctly estimates the depth of these vehicles, as shown in the green close-up. \eloi{possible to check if there are lidar points falling on the car?}
\label{fig:teaser:infinite_depth}
}
\end{subfigure}
\caption{\textbf{Illustration of selected strengths of LiDARTouch over depth depth completion (\emph{left}) and self-supervised monocular depth estimation methods (\emph{right}).}
\eloi{add other points green points of LiDARTouch for other number of beams}
\label{fig:teaser}
}
\end{figure*}


==> tables/interval_evals_RMSE.tex <==
\begin{table*}[!h]
\centering
    \begin{tabular}{@{} l *{8}{@{\hspace{0.2cm}}c} @{}}
    \toprule
    \textbf{Model} & \fz{0.001-10.0} & \fz{10.0-20.0} & \fz{20.0-30.0} & \fz{30.0-40.0} & \fz{40.0-50.0} & \fz{50.0-60.0} & \fz{60.0-70.0} & \fz{70.0-80.0} \\
    \hline
    \imagealone$\PoseNet\imu$ & 0.448 & 0.913 & 2.123 & 3.873 & 4.325 & 5.918 & 5.195 & 3.669 \\
    \imagesparselidar$_\subTouch$ & 0.281 & \textbf{0.446} & \textbf{1.330} & \textbf{2.457} & 3.412 & 3.554 & 3.853 & 3.595 \\
    \ssSD & 0.354 & 0.576 & 1.800 & 2.625 & 3.521 & 3.538 & 4.260 & 4.135 \\ 
    \ssACMNet & \textbf{0.259} & 0.511 & 1.638 & 2.686 & \textbf{3.304} & \textbf{2.777} & 3.937 & 3.903 \\
    \ssNLSPN & 0.324 & 0.665 & 2.339 & 3.054 & 3.474 & 3.205 & \textbf{3.234} & \textbf{3.409} \\
    \bottomrule
    \end{tabular}
    \caption{\label{tab:intervals}\textbf{Evaluation by intervals of 10m} \fontsize{9}{0}{\selectfont here we evaluate the different models for the \textbf{RMSE} metric by intervals of 10 meters up to 80 meters} \eloi{je suis d'avis de ne pas mettre ce tableau, à voir avec les autres}
    }
\end{table*}

==> tables/moving_objects_eval.tex <==
\begin{table}[!h]
\centering
    \caption{\label{tab:moving_objects_eval}\textbf{Influence of LiDAR on moving objects depth estimation} \fontsize{9}{0}{\selectfont as described in \todo{REF}. The evaluation is done using the networks and losses as respectively described in \todo{ref arch} and \todo{ref loss}.  Methods with the prefix ``Ad.'' stands for self-supervised adapted models. All the metrics are computed raw, \ie without ground-truth rescaling.}
    }
    \begin{tabular}{@{} l *{4}{@{\hspace{0.2cm}}c} @{}}
    \toprule
    \textbf{Model} & \fz{Abs Rel} & \fz{Sq Rel} & \fz{RMSE} & $\delta<1.25$ \\
    \hline
    \imagealone$\PoseNet\imu$  & 0.220 & 3.414 & 8.849 & 0.685 \\
    \imagesparselidar$\PnP\selflid$ & 0.106 & 1.116 & 4.895 & 0.896 \\
    \ssSD & 0.123 & 1.099 & 4.744 & 0.882 \\ 
    \ssACMNet & 0.095 & 0.861 & 4.239 & 0.917 \\
    \ssNLSPN & 0.129 & 1.642 & 5.554 & 0.863 \\
    \ssGuideNet & 0.321 & 13.778 & 14.135 & 0.821 \\
    \bottomrule
    \end{tabular}
\end{table}

==> tables/s2d_comparison.tex <==
\begin{table}[]
\addtolength{\tabcolsep}{-4pt}
\centering
\caption{\textbf{Comparison against S2D \citep{selfsup_sparse_to_dense}} on the Depth Completion val set \citep{sparsity_invariant_cnns}. All models are self-supervised ($P$+$L_4$) and use 4-beam LiDAR in input ($\mathcal{I}$+$\mathcal{L}^4$). For ``S2D~\citep{selfsup_sparse_to_dense}'' the result comes from the figure 6b of their paper.}
%
\resizebox{\linewidth}{!}{
\begin{tabular}{@{}crccccc@{}}
\toprule
& \textbf{Network} & \fzz{Multi-view} & \fzz{Abs Rel\,$\downarrow$} & \fzz{Sq Rel\,$\downarrow$} & \fzz{RMSE\,$\downarrow$} & \fzz{$\delta<1.25$\,$\uparrow$}  \\
\hline
& {\footnotesize \ssACMNet} & Yes  & 0.063 & 0.318 & 2.71 & 0.965 \\
& {\footnotesize \ssSD} & Yes & 0.065 & 0.359 & 2.972 & 0.955 \\
& {\footnotesize S2D re-implementation} & No  & 0.088 & 0.438 & 3.246 & 0.940 \\
& {\footnotesize S2D}~\citep{selfsup_sparse_to_dense} & No & - & - & $>$4.0 & - \\
\bottomrule
\end{tabular}
}
\label{tab:s2d_comparison}
\end{table}


==> tables/scaling_evaluation.tex <==

\begin{table}[!h]
\centering
    \caption{\label{tab:scaling}\textbf{Influence of LiDAR on global scale estimation} \fontsize{9}{0}{\selectfont as described in \todo{REF}. The evaluation is done using the networks and losses as respectively described in \todo{ref arch} and \todo{ref loss}. Rows with the symbol "-" indicates that the network is unable to converge (the depth estimation is uniform). All the metrics are computed raw, \ie without ground-truth rescaling. The model \imagealone$\PnP$* use a learning rate of $1e-5$ with a warmup of 1 epoch.}
    }
    \begin{tabular}{@{} l *{4}{@{\hspace{0.2cm}}c} @{}}
    \toprule
    \textbf{Model} & \fz{Abs Rel} & \fz{Sq Rel} & \fz{RMSE} & $\delta<1.25$ \\
    \hline
    \imagealone$\PoseNet$  & 0.990 & 15.338 & 19.117 & 0. \\
    %\imagealone$\PoseNet\imu$  & 0.125 & 0.904 & 5.006 & 0.832 \\
    \imagealone$\PoseNet\imu$ & 0.110 & 0.729 & 4.565 &  0.862 \\
    \imagealone$\PnP$  & - & - & - & - \\
    \imagealone$\PnP$*  & 0.134 & 0.920 & 4.931 & 0.821 \\
    \imagesparselidar$\PnP$ & - & - & - & - \\
    \imagesparselidar$\PoseNet\selflid$ & \todo{} & - & - & - \\ 
    \imagesparselidar$\PoseNet\imu$ & 6.335 & 442.378 & 65.500 & 0.009 \\ 
    \imagesparselidar$\PoseNet\imuAndlid$ & 0.052 & 0.347 & 3.169 & 0.959 \\ 
    \imagesparselidar$\PnP\selflid$ & 0.047 & 0.267 & 2.696 & 0.969 \\ 
    \bottomrule
    \end{tabular}
\end{table}

==> tables/supervision_overview.tex <==
\begin{table*}[t]
\setlength\tabcolsep{0pt} % make LaTeX figure out width of inter-column spaces
\centering
\caption{\textbf{High-level comparison between the LiDARTouch framework and pre-existing approaches.} 
%\eloi{Multiple source views, what is it? Did we talk about it? Mention somewhere.}\flo{It is defined in the L$_\textit{photo}$ presentation, it is the use of multiple source view with min strategy to handle occlusion/deoclusion. S2D use one random view drawn from 6 temporal neighbors.} \eloi{ok, it is a lower-lever details wrt other columns of the table. Two options: option 1: we keep it in the table and we must stress more this difference (eg in the Related work when comparing with S2D, and with an analysis/discussion on why having multiple views is good in the experiment section). option 2: remove it from the table (but we would have less differences with s2d then, which is not ideal)}. 
Inputs of the depth network always involve the image noted $\mathcal{I}$, along with the optional sparse 4-beam or dense 64-beam LiDAR point clouds, respectively noted $\mathcal{L}^{4}$ and $\mathcal{L}^{64}$.
The supervision involves a photometric reconstruction \emph{P} solely, or combined with a LiDAR reconstruction with either the ground-truth \emph{L}$_\textit{gt}$ or with a self-reconstruction of the sparse or dense LiDAR  signal, respectively noted with \emph{L}$_{4}$ or \emph{L}$_{64}$.
\label{tab:supervision_overview}
}
\resizebox{\textwidth}{!}{%
\begin{tabular}{r@{\hspace{0.5cm}}lccccc}
\toprule
\textbf{Framework} & \parbox{1.2cm}{Input} & \parbox{2.6cm}{\centering Ground-truth \\ depth supervision} & \parbox{2.5cm}{\centering LiDAR\\ self-supervision} & \parbox{2.3cm}{\centering Photometric reconstruction}  & \parbox{2.5cm}{\centering Pose\\ estimation}  & \parbox{2.2cm}{\centering Multiple \\ source views}\\
\hline
Monodepth2~\citep{monodepth2} & $\mathcal{I}$ & \xmark & \xmark & \emph{P} & Pose Net. & \cmark \\
DORN~\citep{DORN} & $\mathcal{I}$ & \emph{L}$_\textit{gt}$ & \xmark & \xmark & \xmark & \xmark \\
ACMNet~\citep{ACMNet} & $\mathcal{I}$+$\mathcal{L}^{64}$ & \emph{L}$_\textit{gt}$ & \xmark & \xmark & \xmark & \xmark \\
NLSPN~\citep{non_local_spatial_propagation} & $\mathcal{I}$+$\mathcal{L}^{64}$ & \emph{L}$_\textit{gt}$ & \xmark & \xmark & \xmark & \xmark \\
S2D~\citep{selfsup_sparse_to_dense} & $\mathcal{I}$+$\mathcal{L}^{64}$ & \xmark & \emph{L}$_{64}$ & \emph{P} & PnP & \xmark \\
LiDARTouch (ours) & $\mathcal{I}$+$\mathcal{L}^{4}$ & \xmark & \emph{L}$_{4}$ & \emph{P} & PnP & \cmark \\
\bottomrule
\end{tabular}
}
\end{table*}


%\textbf{Framework}                           & \parbox{2.3cm}{\centering Photometric reconstruction}  & \parbox{2.2cm}{\centering Multiple \\ source views} & \parbox{2.6cm}{\centering Ground-truth \\ depth supervision}  & \parbox{2.5cm}{\centering LiDAR\\ self-supervision} & \parbox{1.4cm}{\centering \# LiDAR\\ beams} & \parbox{2.5cm}{\centering Pose\\ estimation} \\
%\hline
%Monodepth2~\citep{monodepth2} & \cmark & \cmark & \xmark & \xmark & 0 & Network             \\
%ACMNet~\citep{ACMNet} & \xmark & \xmark & \cmark & \xmark & 64 & None                       \\
%NLSPN~\citep{non_local_spatial_propagation} & \xmark & \xmark & \cmark & \xmark & 64 & None \\
%S2D~\citep{selfsup_sparse_to_dense} & \cmark & \xmark & \xmark & \cmark & 64 & PnP          \\
%LiDARTouch (ours) & \cmark & \cmark & \xmark & \cmark & 4 & Network/PnP                     \\
